Efficient Measurement on Programmable Switches Using Probabilistic Recirculation

Programmable network switches promise flexibility and high throughput, enabling applications such as load balancing and traffic engineering. Network measurement is a fundamental building block for such applications, including tasks such as the identification of heavy hitters (largest flows) or the detection of traffic changes. However, high-throughput packet processing architectures place certain limitations on the programming model, such as restricted branching, limited capability for memory access, and a limited number of processing stages. These limitations restrict the types of measurement algorithms that can run on programmable switches. In this paper, we focus on the RMT programmable high-throughput switch architecture, and carefully examine its constraints on designing measurement algorithms. We demonstrate our findings while solving the heavy hitter problem. We introduce PRECISION, an algorithm that uses \emph{Probabilistic Recirculation} to find top flows on a programmable switch. By recirculating a small fraction of packets, PRECISION simplifies the access to stateful memory to conform with RMT limitations and achieves higher accuracy than previous heavy hitter detection algorithms that avoid recirculation. We also analyze the effect of each architectural constraint on the measurement accuracy and provide insights for measurement algorithm designers.

==> backup_figures.tex <==

\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/associativity/tests2.1.2018.caida.associativity.out/AverageOnArrivalMSE.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/associativity/tests2.1.2018.UCLA.associativity.out/AverageOnArrivalMSE.pdf}} & 
		\subfloat[Zipf1 - TODO run!]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/associativity/tests2.1.2018.caida.associativity.out/AverageOnArrivalMSE.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/associativity/tests2.1.2018.caida.associativity.out/legend.png}}          
	\caption{\label{fig:assoctive}Effect of associativity on the overall estimation error.}
\end{figure*}
\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/associativity/tests2.1.2018.caida.associativity.out/recallVsCounters-128.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/associativity/tests2.1.2018.UCLA.associativity.out/recallVsCounters-128.pdf}} & 
		\subfloat[Zipf1 - TODO run!]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/associativity/tests2.1.2018.caida.associativity.out/recallVsCounters-128.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/associativity/tests2.1.2018.caida.associativity.out/legend.png}}          
	\caption{\label{fig:assocTopK}Associativity and the number of counters to identify the top 128 flows. }
\end{figure*}



\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/delay/tests25.12.out.delay.caida/AverageOnArrivalMSE.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/delay/tests25.12.out.delay.UCLA/AverageOnArrivalMSE.pdf}} & 
		\subfloat[Zipf1]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/delay/tests25.12.out.delay.zipf1.0/AverageOnArrivalMSE.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/delay/tests25.12.out.delay.caida/legend.png}}          
	\caption{\label{fig:packetFE}Effect of packet delay on the overall estimation error.}
\end{figure*}
\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/delay/tests25.12.out.delay.caida/recallVsCounters-128.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/delay/tests25.12.out.delay.UCLA/recallVsCounters-128.pdf}} & 
		\subfloat[Zipf1]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/delay/tests25.12.out.delay.zipf1.0/recallVsCounters-128.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/delay/tests25.12.out.delay.caida/legend.png}}          
	\caption{\label{fig:packetTopK}Packet delay and the number of counters to identify the top 128 flows. }
\end{figure*}

 
 
\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/initValue/tests25.12.out.initVal.caida/AverageOnArrivalMSE.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/initValue/tests25.12.out.initVal.UCLA/AverageOnArrivalMSE.pdf}} & 
		\subfloat[Zipf1]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/initValue/tests25.12.out.initVal.zipf1.0/AverageOnArrivalMSE.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/initValue/tests25.12.out.initVal.caida/legend.png}}          
	\caption{\label{fig:initFE}Frequency estimation accuracy and initial value. }
\end{figure*}
\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/initValue/tests25.12.out.initVal.caida/recallVsCounters-128.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/initValue/tests25.12.out.initVal.UCLA/recallVsCounters-128.pdf}} & 
		\subfloat[Zipf1]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/initValue/tests25.12.out.initVal.zipf1.0/recallVsCounters-128.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/initValue/tests25.12.out.initVal.caida/legend.png}}          
	\caption{\label{fig:initTopK}Top 128 accuracy and initial value. }
\end{figure*}
\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/initValue/tests25.12.out.initVal.caida/averages/AvgConvergence--128-using-512.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/initValue/tests25.12.out.initVal.UCLA/averages/AvgConvergence--128-using-512.pdf}} & 
		\subfloat[Zipf1]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/initValue/tests25.12.out.initVal.zipf1.0/averages/AvgConvergence--128-using-512.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/initValue/tests25.12.out.initVal.caida/legend.png}}          
	\caption{\label{fig:InitConverge}Convergence of initial values for finding top 128 with 512 counters. }
\end{figure*}



\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/compromises/tests25.12.out.compromises.caida/AverageOnArrivalMSE.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/compromises/tests25.12.out.compromises.UCLA/AverageOnArrivalMSE.pdf}} & 
		\subfloat[Zipf1 - TODO run!]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/compromises/tests25.12.out.compromises.zipf1.0/AverageOnArrivalMSE.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/compromises/tests25.12.out.compromises.caida/legend.png}}          
	\caption{\label{fig:RestrictFE}Frequency estimation accuracy and restricted sampling. }
\end{figure*}
\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/compromises/tests25.12.out.compromises.caida/recallVsCounters-128.pdf}} &    
		\subfloat[UCLA\label{topKUCLA}]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/compromises/tests25.12.out.compromises.UCLA/recallVsCounters-128.pdf}} & 
		\subfloat[Zipf1]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/compromises/tests25.12.out.compromises.zipf1.0/recallVsCounters-128.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/compromises/tests25.12.out.compromises.caida/legend.png}}          
	\caption{\label{fig:RestrictTopK}Top 128 accuracy and restricted sampling. }
\end{figure*}
\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/Comparison/tests25.12.out.caida/AverageOnArrivalMSE.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/Comparison/tests25.12.out.UCLA/AverageOnArrivalMSE.pdf}} & 
		\subfloat[Zipf1]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/Comparison/tests25.12.out.zipf1.0/AverageOnArrivalMSE.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/Comparison/tests25.12.out.caida/legend.png}}          
	\caption{\label{fig:comparativeFE}Comparative evaluation of the frequency estimation problem. }
\end{figure*}
\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[Caida]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/Comparison/tests25.12.out.caida/recallVsCounters-128.pdf}} &    
		\subfloat[UCLA]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/Comparison/tests25.12.out.UCLA/recallVsCounters-128.pdf}} & 
		\subfloat[Zipf1]{\includegraphics[width = 0.66\columnwidth]
			{simulations/new/Comparison/tests25.12.out.zipf1.0/recallVsCounters-128.pdf}}    
	\end{tabular}    
	\centering{\includegraphics[width = \columnwidth]
		{simulations/new/Comparison/tests25.12.out.caida/legend.png}}          
	\caption{\label{fig:comparativeTopK}Comparative evaluation for the top Top-128 problem. }
\end{figure*}



